Towards Zero-Overhead Adaptive Indexing in Hadoop

Several research works have focused on supporting index access in MapReduce systems. These works have allowed users to significantly speed up selective MapReduce jobs by orders of magnitude. However, all these proposals require users to create indexes upfront, which might be a difficult task in certain applications (such as in scientific and social applications) where workloads are evolving or hard to predict. To overcome this problem, we propose LIAH (Lazy Indexing and Adaptivity in Hadoop), a parallel, adaptive approach for indexing at minimal costs for MapReduce systems. The main idea of LIAH is to automatically and incrementally adapt to users' workloads by creating clustered indexes on HDFS data blocks as a byproduct of executing MapReduce jobs. Besides distributing indexing efforts over multiple computing nodes, LIAH also parallelises indexing with both map tasks computation and disk I/O. All this without any additional data copy in main memory and with minimal synchronisation. The beauty of LIAH is that it piggybacks index creation on map tasks, which read relevant data from disk to main memory anyways. Hence, LIAH does not introduce any additional read I/O-costs and exploit free CPU cycles. As a result and in contrast to existing adaptive indexing works, LIAH has a very low (or invisible) indexing overhead, usually for the very first job. Still, LIAH can quickly converge to a complete index, i.e. all HDFS data blocks are indexed. Especially, LIAH can trade early job runtime improvements with fast complete index convergence. We compare LIAH with HAIL, a state-of-the-art indexing technique, as well as with standard Hadoop with respect to indexing overhead and workload performance.

==> formula.tex <==


$$t_{indexRead} = (sel \cdot t_{fS} + t_{iA})\cdot \#indBl$$
$$t_{fullRead} = t_{fS} \cdot (\#bl -\#indBl)$$
$$t_{indexing} = t_{iO} \cdot oR \cdot (\#bl -\#indBl) $$
$$t_{job} = t_{fullRead} + t_{indexing} + t_{indexRead}  + t_{jobO}$$

Where $oR$ is the offer rate , $t_{iO}$ the indexing overhead , $t_{fS}$ the full scan time, $t_{iA}$ the time to access the index on disk and  $t_{jobO}$ the overhead involved in executing an empty MapReduce job.

==> indexstore.tex <==
%!TEX root = main.tex
\subsection{Storing the Indexed Blocks}
After the adaptive indexer thread performed the in-memory index creation it stores the resulting index block in HDFS. 
The index block is similar to the original block and consists of the block metadata header, the index root node and the reordered data. If all attributes were loaded from the original block, the index is logically a full replica of the block stored in a different sort order.  

We store this block in a separate HDFS file with replication factor one, it is very likely that the file will be created on the same data node as the original block. 
To uniquely identify an index file we follow a naming convention, that contains the block identifier and the id of the main index attribute.
Additionally to storing the index file we inform the Namenode about the new index. 

\subsection{Accessing Indexed Blocks}


\subsection{Adaptive HAIL Scheduling}
In the beginning of a map reduce job, the input is split into so called input splits. Those splits are then processed in individual tasks by task trackers. In standard Hadoop one input split corresponds to one HDFS block, this is done to allow for improved data locality and reduce the performance impact of failures. If a task fails only one block needs to be re-read. In case of index access it is not really necessary to re-read a whole block, but only the needed data. As shown in the HAIL paper, the map reduce scheduling overhead can be reduced drastically by combining many blocks that are stored on the same data node into a single split. To not endanger failover properties this should only be done with blocks that can be processed, or re-processed, very fast, this is the case for blocks on which an index exists.

Our new scheduling strategy, \emph{adaptive HAIL scheduling} , combines all blocks that have an useful index on the same data node to a singe input split, but keeps all blocks that have no index in separate input splits, as normal Hadoop would do.


==> ssd.tex <==
%!TEX root = main.tex
\section{\hail using Solid-State Drives}
\label{appendix:ssd}

\color{red}
{\bf TODO: insert SSD results (not sure we require this section)}
\color{black}

%For one of the experiments, we also inserted an additional SSD with a capacity of 250 GB into all ten nodes. 

%while the SSDs are formatted using ext4.


\begin{figure}[!h]
%\vspace*{-0.4cm}
\centering\includegraphics[width=\linewidth]{graphics/offer_old_pavlo_ssd_256.pdf}
%\vspace*{-0.5cm}
\caption{Offer rate impact on a sequence of eleven queries touching different ranges of the same attribute with the same selectivity on pavlo dataset, with solid state disks.}
\label{figure:offerPavloSSD}
%\vspace*{-0.3cm}
\end{figure}


